Finite-data error bounds for Koopman-based prediction and control

The Koopman operator has become an essential tool for data-driven approximation of dynamical (control) systems, e.g., via extended dynamic mode decomposition. Despite its popularity, convergence results and, in particular, error bounds are still scarce. In this paper, we derive probabilistic bounds for the approximation error and the prediction error depending on the number of training data points; for both ordinary and stochastic differential equations while using either ergodic trajectories or i.i.d. samples. We illustrate these bounds by means of an example with the Ornstein-Uhlenbeck process. Moreover, we extend our analysis to (stochastic) nonlinear control-affine systems. We prove error estimates for a previously proposed approach that exploits the linearity of the Koopman generator to obtain a bilinear surrogate control system and, thus, circumvents the curse of dimensionality since the system is not autonomized by augmenting the state by the control inputs. To the best of our knowledge, this is the first finite-data error analysis in the stochastic and/or control setting. Finally, we demonstrate the effectiveness of the bilinear approach by comparing it with state-of-the-art techniques showing its superiority whenever state and control are coupled.

==> sections/control_estimate_backup.tex <==
\section{Extension to control systems}
\label{sec:control}

\MS{\noindent In this section, we derive probabilistic bounds on the approximation error of controlled SDE systems of the form
\begin{align}\label{e:sde_control}
\text{d}X_t = \left(F(X_t)+   \sum_{i=1}^{n_c} G_i(X_t)u_i \right)\text{d}t  + \sigma(X_t) \,\text{d}W_t,
\end{align}
with input $u\in\mathbb{R}^{n_c}$ and state $X_t\in\XX$, where $F:\XX\to\mathbb{R}^n$ and $G_i: \XX\to\mathbb{R}^{n}$, $i = 1,\ldots,n_c$, are locally Lipschitz-continuous vector fields. In the deterministic case $\sigma\equiv 0$ the controlled SDE reduces to the control-affine ODE system
\begin{align}\label{e:controlaffine}
\dot{x} = F(x) + \sum_{i=1}^{n_c} G_i(x)u_i, \qquad x(0)=x_0.
\end{align}
We will describe how one can apply the bounds on the generators of autonomous (SDE) systems obtained in Section~\ref{sec:SDE} in order to obtain bounds for prediction of control systems, either for i.i.d.\ or ergodic sampling.

%In the ergodic setting, all considerations in this section are also applicable to controlled SDE systems, cf.\ Section~\ref{sec:SDE}, i.e.,
%with \MS{straightforward } modifications. We will stick to the deterministic case for the sake of readability and provide a numerical example of a controlled SDE in Section~\ref{sec:examples}.



Central in this part is the fact that the Koopman generators for control-affine systems are control-affine. More precisely, if $\mathcal{L}^{\bar{u}}$ denotes the Koopman generator for a control-affine system with constant control $\bar{u}\in \mathbb{R}^{n_c}$ and $\bar u = \sum_{i=1}^{r}\alpha_i \bar u_i$ is a linear combination of constant controls $\bar u_i\in\R^{n_c}$, we have
\begin{align}\label{e:gen_ca}
%\mathcal{L}^{\alpha_1\bar{u}_1 + \alpha_2\bar{u}_2} = \mathcal{L}^0 + \alpha_1\left(\mathcal{L}^{\bar{u}_1} -  \mathcal{L}^0\right)+ \alpha_2\left(\mathcal{L}^{\bar{u}_2} -  \mathcal{L}^0\right)
\calL^{\bar u} = \calL^0 + \sum_{i=1}^{n_c}\alpha_i\big(\calL^{\bar u_i} - \calL^0\big).
\end{align}
%for any $\alpha_1,\alpha_2\in\mathbb{R}$ and $\bar{u}_1,\bar{u}_2\in\mathbb{R}^{n_c}$.
This easily follows from the representation \eqref{e:repL} of the Koopman generator, see also \cite[Theorem 3.2]{Peitz2020} for the special (deterministic) case $\sigma\equiv 0$.

We will utilize this property to invoke our results from Section~\ref{sec:SDE} to approximate the Koopman generator corresponding to basis elements of the control space, that is, $\mathcal{L}^{e_i}$, $i=1,\ldots,n_c$, and $\mathcal{L}^0$ corresponding to the drift term to form a bilinear control system in the observables.
%In the following, $\mathcal{O}$ will serve as a placeholder for a Hilbert space of observables $\psi:\mathbb{X}\to\mathbb{R}$ and will be specified later.



Analogously to Assumption~\ref{as:data} we have the following two cases for the collected data and the underlying measure.
\begin{assumption}
	\label{as:control_data}
	Let either of the following hold:
	\begin{itemize}
		\item[(iid)] The data for each autonomous system with control $u=e_i$, $i=0,\ldots,n_c$ is sampled i.i.d.\ from either the normalized Lebesgue measure and contained in a compact forward invariant set $\mathbb{X}_i$ or from an invariant measure $\mu_i$ in the sense of Definition~\ref{def:invariant_measure}.
		\item[(erg)] The data for each autonomous system with control $u=e_i$, $i=0,\ldots,n_c$ satisfies Assumption~\ref{as:data}.(erg), i.e., is drawn from a single ergodic trajectory, the probability measure $\mu_i$ of the resulting autonomous SDE is invariant in the sense of Definition~\ref{def:invariant_measure} and the Koopman semigroup is exponentially stable on $L^2_{\mu_i,0}(\mathbb{X}_i)$.
	\end{itemize}
\end{assumption}
\noindent 
In \textup{\cite{ZhanZuaz21}} the authors sample i.i.d.\ data from the Lebesgue measure and that the set $\mathbb{X}$ is compact and forward invariant with respect to the dynamics and also comment on weakening the assumption of forward invariance of $\mathbb{X}$, cf.\ the discussion in \textup{\cite[Section 3.2]{ZhanZuaz21}}. 

 In the following, we set $\mathcal{O}_i = L^2_{\mu_i}(\mathbb{X}_i)$, $i=1,\ldots,n_c$, and consider the generators $\calL^{e_i}$ in these spaces, respectively. Further, let $\psi_1,\ldots,\psi_N : \mathbb X\to\R$ be $N$ linearly independent observables whose span $\mathbb V = \linspan\{\psi_1,\ldots,\psi_N\}$ satisfies
\begin{align}\label{e:intersec}
\mathbb{V} \subset D(\mathcal{L}^{e_0})\cap D(\mathcal{L}^{e_1})\cap \ldots \cap D(\mathcal{L}^{e_{n_c}}),
\end{align}
where $e_i$, $i=1,\ldots,n_c$, denote the standard basis vectors of $\mathbb{R}^{n_c}$ and $e_0 := 0$. We now discuss two cases of sampling, one corresponding to the approach of Section \ref{sec:SDE} and one to the standard case of i.i.d.\ sampling as in \cite{ZhanZuaz21}.

As the original system and the Koopman generator are control affine, the remainder of this section is split up into two parts. First, we derive error estimates corresponding to autonomous systems driven by $n_c+1$ constant controls. Second, we use these estimates and control affinity to deduce a result for general controls.

%\medskip
%\noindent\textbf{Ergodic sampling.}

% A sufficient condition for the intersection on the right-hand side of \eqref{e:intersec} to be non-empty is that the sets contained in the respective domains in Remark~\ref{rem:domain} have non-trivial intersection. This, of course, depends on the measures $\mu(0),\ldots,\mu(e_{n_c})$.

%\medskip
%\noindent\textbf{I.i.d.\ sampling.} 

%Here, we assume that for each autonomous SDE \eqref{e:sde_control} on $\XX = \R^n$ with constant control $u=e_i$, $i=0,\ldots,n_c$, there is an invariant measure $\mu_i$, cf.\ Assumption~\ref{assumption:invariant_measure}. Then, we set $\mathcal{O}_i = L^2_{\mu_i}(\mathbb{X})$, $i=1,\ldots,n_c$, and consider the generators $\calL^{e_i}$ in these spaces, respectively.

%Here, we consider the  SDE \eqref{e:sde_control} on a compact set $\mathbb{X}\subset\R^n$ and assume that the samples are drawn independently and uniformly from $\mathbb X$, i.e., with respect to $\mu$. In this case, we set $\mathcal{O}=L^2(\mathbb{X})$.
% and we can choose any finite subset of functions in the set $\left\{\psi\in \mathcal{O} \, | \, \nabla \psi \in \mathcal{O} \right\}$ for our basis of observables spanning $\mathbb{V}$.


%In view of the previous remark, and in order to ensure well-definedness of the observables and the corresponding Koopman operator, we have to assume that the sampled data points $x_k$, $k=0,\ldots m-1$, are contained in the set $\mathbb{X}$.

%In the following, by $\mathcal{L}^{e_i}_\mathbb{V}$ we again denote the projection of the Koopman generator $\mathcal{L}^{e_i}$ onto the finite dimensional space $\mathbb{V}$.
\noindent In accordance with the notation in Section \ref{sec:SDE} we define $\calL_{\mathbb V}^{e_i} := P_{\mathbb V}\calL^{e_i}|_{\mathbb V}$ and also use this symbol to denote the matrix representation of this linear operator w.r.t.\ to the basis $\{\psi_1,\ldots,\psi_N\}$ of $\mathbb V$. Its approximation based on the data $x_0,\ldots,x_{m-1}\in\mathbb X$ will be denoted by $\tilde\calL_m^{e_i}$.

\begin{proposition}\label{p:single_estimate}
Let $i \in \{0,\ldots,n_c\}$ be given and Assumption~\ref{as:control_data} hold.
%one of the following two conditions holds:
%\begin{enumerate}
%\item \braces{$\XX=\R^n$, $\sigma\neq 0$} The autonomous SDE \eqref{e:sde_control} with constant control $u\equiv e_i$ gives rise to an invariant measure in the sense of Assumption~\ref{assumption:invariant_measure} such that also Assumption~\ref{as:data}.(erg) holds.
%\item \braces{$\XX$ compact, $\sigma\equiv 0$} The samples are drawn i.i.d.\ from the uniform distribution on $\mathbb X$.
%\end{enumerate}
Then, for any pair consisting of a desired error bound $\varepsilon > 0$ and a probabilistic tolerance $\delta\in (0,1)$, there is a number of data points $m_i$ such that for any $m \geq m_i$, we have the estimate
\begin{align*}
\mathbb{P}\big( \| \LV^{e_i}-\tL^{e_i}\|_F\leq \varepsilon\big) \geq 1-\delta.
\end{align*}
The minimal amount of data $m_i$ is given by the formulas of Theorem~\ref{t:generatorestimate}.
%If Assumption~\textup{1} holds, $m_i$ is given by the formulas of Theorem~\rmref{t:generatorestimate}, i.e.\ Condition \eqref{eq:ineq_m}. If Assumption~\textup{2} holds and the samples are contained in $\mathbb{X}$, $m_i$ is given by the estimate in \textup{\cite[Proposition 4.2]{ZhanZuaz21}}.
\end{proposition}
\begin{proof}
The claim follows immediately from applying Theorem~\ref{t:generatorestimate}.
%In case of Assumption \ref{as:control_data}., the claim follows by applying Theorem~\ref{t:generatorestimate}. In case of Assumption 2, we apply \cite[Proposition 4.2]{ZhanZuaz21} to $\LV^{e_i}$ for $i=0,\ldots,n_c$.
\end{proof}

%In the following, we consider trajectories evolving in the set $\mathbb{X} := \bigcap_{i=0}^{n_c} \mathbb{X}_i$ which is of course not necessarily forward invariant.  In the control context, an assumption of invariance of $\mathbb{X}$ for all autonomous systems corresponding to the constant controls $e_i$, $i=0,\ldots,n_c$, seems very restrictive, which is why we chose not to assume this here. However, the lack of invariance is not an issue if one guarantees that the state is contained in this set via, e.g., stabilization. 




\noindent Having obtained an estimate for the autonomous systems corresponding to the constant controls $e_i, i=0,\ldots n_c$, we can leverage the control affinity of the system to formulate the corresponding results for arbitrary controls. To this end, for any control $u(t) = \sum_{i=1}^{n_c}\alpha_i(t) e_i \in L^\infty(0,T;\mathbb{R}^{n_c})$, we define the projected Koopman generator and its approximation corresponding to the non-autonomous system with control $u$ by
\begin{align*}
\LV^u (t) &:= \LV^0 + \sum_{i=1}^{n_c}\alpha_i(t)\big(\LV^{e_i}-\LV^0\big),\\
\tL^u(t) &:= \tL^0 + \sum_{i=1}^{n_c}\alpha_i(t)\big(\tL^{e_i}-\tL^0\big).
\end{align*}


\begin{theorem}\label{t:coupled_estimate}
Let Assumption~\ref{as:control_data}  hold. 
Then, for any pair consisting of a desired error bound $\tilde\varepsilon > 0$ and probabilistic tolerance $\tilde\delta \in (0,1)$, prediction horizon $T>0$, and control function $u\in L^\infty(0,T;\mathbb{R}^{n_c})$ %such that the solution of \eqref{e:SDE} is contained in $\mathbb{X}$, 
we have
\begin{align*}
\operatorname{ess\,inf}_{t \in [0,T]}\mathbb{P}\big(\|\LV^u(t) - \tL^u(t)\|_F \leq \tilde\varepsilon\big) \geq 1-\tilde\delta,
\end{align*}	
provided that the number~$m$ of data points exceeds $\max_{i=0,\ldots,n_c} m_i$ with $m_i$ defined as in Proposition~\rmref{p:single_estimate} with
$$
\veps = \tfrac{\tilde\varepsilon}{(n_c+1)\left(1  + \sum_{i=1}^{n_c}\|\alpha_i\|_{L^\infty(0,T)}\right)}
\qquad\text{and}\qquad
\delta = 1-\tfrac{\tilde\delta}{n_c+1}.
$$
% there is $m_0 \in \mathbb{N}$ such that for $m\geq m_0$ data points contained in $\mathbb{X}$ we have 
%Further, $m_0$ is given by 
%\begin{align*}
%m &\geq \frac{4C  \xi_{\max}^2 e^{-\omega \Delta_t}}{\eta \lambda_\xi^{\min} (1 - e^{-\omega \Delta_t})^2},
%\end{align*}
%	\begin{align}
%m \geq \frac{2N^2 \max\{\lambda_\xi^{\max},\lambda_\chi^{\max}\}(1 + \eta){\left(\|C^{-1}\| + \tfrac{\varepsilon}{2\|A\|}\right) \|C^{-1}\|}}{ \tfrac{\varepsilon}{2\|A\|}\delta}. 
%\end{align}
%and
%\begin{align}
%m \geq \frac{2N^2 \max\{\lambda_\xi^{\max},\lambda_\chi^{\max}\}(1 + \eta)2\left(\|C^{-1}\|+\tfrac{\varepsilon}{2\|A\|}\right)}{\varepsilon \delta}. 
%\end{align}	
\end{theorem}
\begin{proof}
Again, we omit the subscript of the norm and set $\|\cdot\|=\|\cdot\|_F$.
Using the result of Proposition~\ref{p:single_estimate} and our choice of $m_0$, we have
$$
\mathbb{P}\left( \|\tL^{0}-\LV^0\| \leq \tfrac{\tilde\varepsilon}{(n_c+1)\left(1  + \sum_{i=1}^{n_c}\|\alpha_i\|_{L^\infty(0,T)}\right)}\right) \geq 1-\tfrac{\tilde\delta}{n_c + 1},
$$
and for all $i\in 1,\ldots n_c$
$$
\mathbb{P}\left(\|\LV^{e_i} - \tL^{e_i}\| \leq \tfrac{\tilde\veps}{\left(n_c+1\right)\|\alpha_i\|_{L^\infty(0,T)}}\right) \geq 1- \tfrac{\tilde\delta}{n_c + 1}.
$$
Then we compute for $a.e.\ t\in [0,T]$
\begin{align*}
& \mathbb{P}\left( \| \LV^u(t) -  \tL^u(t) \|\leq \tilde\veps\right)& \\
&\geq \mathbb{P}\left(\left\|\left(1-\sum_{i=1}^{n_c}\alpha_i(t)\right)\left(\LV^0 - \tilde\calL_m^0\right)\right\|+ \sum_{i=1}^{n_c} \left\| \alpha_i(t)\left(\tL^{e_i} - \LV^{e_i}\right)\right\| \leq \tilde\veps\right)\\
&\geq \mathbb{P}\left(\left\|\left(1-\sum_{i=1}^{n_c}\alpha_i(t)\right)\left(\LV^0 - \tilde\calL_m^0\right)\right\| \leq \tfrac{\tilde\veps}{n_c+1}\,\wedge\,
%\bigwedge_{i=1}^{n_c}
\displaystyle\mathop{\mathlarger{\mathlarger{\mathlarger{\forall}}}}_{i=1}^{n_c} : 
\left\|\alpha_i(t) \left(\tL^{e_i} - \LV^{e_i}\right)\right\|
 \leq \tfrac{\tilde\veps}{n_c+1}\right).
\end{align*}
%\red{Auch das verstehe ich nicht (erste Abschaetzung). Es gilt doch
%	\begin{align*}
%		\LV^u(t) -  \tL^u(t)
%		= \left(1-\sum_{i=1}^{n_c}\alpha_i(t)\right)(\calL_V^0 - \tilde\calL_m^0) + \sum_{i=1}^{n_c}\alpha_i(t)(\calL_V^{e_i} - \tilde\calL_m^{e_i})
%\end{align*}}
Next, we use Lemma~\ref{lem:probabilities} from Appendix \ref{ss:technical} with $d = n_c+1$, 
$$
A_0 = \left\{\left\|\left(1-\sum_{i=1}^{n_c}\alpha_i(t)\right)\left(\LV^0 - \tilde\calL_m^0\right)\right\| \leq \tfrac{\tilde\veps}{n_c+1}\right\}
\quad \text{and}\quad
A_i = \left\{ \left\|\alpha_i(t) \left(\tL^{e_i} - \LV^{e_i}\right)\right\| \leq \tfrac{\tilde\veps}{n_c+1}\right\}
$$
for $i=1,\ldots,n_c$. This yields
\begin{align*}
& \mathbb{P}\left( \| \LV^u(t) -  \tL^u(t) \|\leq \tilde\veps\right)& \\
&\geq \mathbb{P}\left( \left\|\left(1-\sum_{i=1}^{n_c}\alpha_i(t)\right)\left(\LV^0 - \tilde\calL_m^0\right)\right\| \leq \tfrac{\tilde\veps}{n_c+1} \right)
%\\&\qquad \qquad+ \sum_{i=1}^{n_c} \mathbb{P}\left( \|\alpha_i(t)\left(\tL^{e_i}-\LV^{{e_i}}\right)\| \leq \tfrac{\tilde\veps}{n_c+1}  \right) - n_c \\
+ \sum_{i=1}^{n_c} \mathbb{P}\left( \|\alpha_i(t)\big(\tL^{e_i}-\LV^{{e_i}}\big)\| \leq \tfrac{\tilde\veps}{n_c+1}  \right) - n_c \\
&\geq \mathbb{P}\left( \|\tL^{0}-\LV^0\| \leq \tfrac{\tilde\veps}{\left(1  + \sum_{i=1}^{n_c} \|\alpha_i\|_{L^\infty(0,T)}\right)(n_c+1)}  \right)
%\\&\qquad + \sum_{i=1}^{n_c} \mathbb{P}\left( \|\tL^{e_i}-\LV^{{e_i}}\| \leq \tfrac{\tilde\veps}{\|\alpha_i\|_{L^\infty(0,T;\mathbb{R})}\left(n_c+1\right)}  \right) - n_c\\
+ \sum_{i=1}^{n_c} \mathbb{P}\left( \|\tL^{e_i}-\LV^{{e_i}}\| \leq \tfrac{\tilde\veps}{\left(n_c+1\right)\|\alpha_i\|_{L^\infty(0,T)}}  \right) - n_c\\
&\geq 1-\tfrac{\tilde\delta}{n_c+1} + \sum_{i=1}^{n_c} \left(1-\tfrac{\tilde\delta}{n_c+1}\right) - n_c = 1-\tilde\delta.
\end{align*}
Taking the essential infimum yields the result.
\end{proof}

\noindent Again, similar as in the previous section, we obtain a bound on trajectories via Gronwall, if the state response is contained in $\mathbb{X}$. %The latter could be omitted, if one assumes forward invariance of the set $\mathbb{X}$ for all controls, cf.\ Remark~\ref{rem:fi}.

\begin{corollary}\label{c:control_trajectory}
Let Assumption~\ref{as:control_data}  hold. Let $T,\veps>0$ and $\delta\in (0,1)$, $z_0\in \mathbb{R}^N$ and $u\in L^\infty(0,T;\mathbb{R}^{n_c})$. %such that the solution of \eqref{e:SDE} is contained in $\mathbb{X}$. 
Then there is $m_0\in \mathbb{N}$ such that for $m\geq m_0$ %data points contained in $\mathbb{X}$, 
the solutions $z,\tilde{z}$ of
%for $m_0 \in \mathbb{N}$ as given in Theorem~\ref{t:coupled_estimate} and $m\geq m_0$ data points contained in $\mathbb{X}$, the solutions $z,\tilde{z}$ of
\begin{align*}
&&\dot{z}(t) &= \LV^u(t)z &&z(0)=z_0\\
&&\dot{\tilde{z}}(t) &= \tL^u(t)\tilde{z} &&\tilde{z}(0)={z}_0
\end{align*}
satisfy
\begin{align*}
\min_{t\in [0,T]}\mathbb{P}\big( \|z(t)-\tilde{z}(t)\|_2 \leq \varepsilon\big) \geq 1-\delta.
\end{align*}
\end{corollary}
\begin{proof}
See Appendix~\ref{s:errorbound_traj}.
\end{proof}

\noindent As in Corollary~\ref{c:trajest}, $m_0$ can explicitly be computed by combining Theorem~\ref{t:coupled_estimate} with the constants in Gronwalls inequality.

We conclude this section with a final corollary regarding the optimality of the solution obtained using an error-certified Koopman model. To this end, we consider the optimal control problem
\begin{equation}\label{eq:OCP_full}
\begin{aligned}
&\min_{u\in L^\infty(0,T;\mathbb{R}^{n_c})} J(x)\\
\mbox{s.t.}\qquad \dot{x} &= F(x) + \sum_{i=1}^{n_c} G_i(x)u_i, \qquad x(0)=x_0.
\end{aligned}
\end{equation}
In what follows, we compare the optimal value of the Koopman representation of \eqref{eq:OCP_full} projected onto the subspace of observables $\mathbb{V}$ with initial datum $z_0 = \Psi (x_0)$
\begin{equation}\label{eq:OCP_full_Koop}
\begin{aligned}
&\min_{\alpha\in L^\infty(0,T;\mathbb{R}^{n_c})} J(P(z))\\
\mbox{s.t.}\qquad \dot{{z}}(t) &= \left[\LV^0 + \sum_{i=1}^{n_c}\alpha_i(t)\left(\LV^{e_i}-\LV^0\right)\right]{z}(t), \qquad {z}(0)={z}_0,
\end{aligned}
\end{equation}
to the optimal value of the surrogate-based control problem:
\begin{equation}\label{eq:OCP_surrogate}
\begin{aligned}
&\min_{\tilde \alpha\in L^\infty(0,T;\mathbb{R}^{n_c})} J(P(\tilde{z}))\\
\mbox{s.t.}\qquad \dot{\tilde{z}}(t) &= \left[\tL^0 + \sum_{i=1}^{n_c}\tilde\alpha_i(t)\left(\tL^{e_i}-\tL^0\right)\right]\tilde{z}(t), \qquad \tilde{z}(0)={z}_0,
\end{aligned}
\end{equation}
where $P$ maps a trajectory of observables to a trajectory in the state space, which in practice is frequently realized by including the coordinates of the identity function in the dictionary~$\Psi$ of observables.%contained in $\mathbb{V}$, i.e., $\Phi (z_1,\ldots,z_N) = \sum_{i=1}^N z_i \psi_i.$%

%\red{$P$ sollte hier meiner Meinung nach einfach der Isomorphismus $\Phi : \R^N\to\mathbb V$ sein und kann somit als Einbettung $\R^N\to L^2_\mu$ gesehen werden -- also genau das Gegenteil einer Projektion.}

\begin{corollary}\label{c:control_problem}
Let $T,\veps>0$, $\delta\in (0,1)$, $z_0\in \mathbb{R}^N$, let $J$ be Lipschitz continuous and let Assumption~\ref{as:control_data}  hold.
Furthermore, let $(z^*,\alpha^*)$ be an optimal solution of problem \eqref{eq:OCP_full_Koop}. Then there is $m_0\in \mathbb{N}$ such that for $m\geq m_0$ data points contained in $\mathbb{X}$, there exists a tuple $(\tilde{z},\tilde{\alpha})$ which is feasible for \eqref{eq:OCP_surrogate} such that %if the state of the dynamics of \eqref{eq:OCP_full} is contained in $\mathbb{X}$
\[
\mathbb{P}\big(|J(P(\tilde{z}))- J(P(z^*))| \leq \varepsilon\big) \geq 1-\delta.
\]
\end{corollary}}
